Storage Control for Carbon Emission Reduction: Opportunities and Challenges

Storage is vital to power systems as it provides the urgently needed flexibility to the system. Meanwhile, it can contribute more than flexibility. In this paper, we study the possibility of utilizing storage system for carbon emission reduction. The opportunity arises due to the pending implementation of carbon tax throughout the world. Without the right incentive, most system operators have to dispatch the generators according to the merit order of the fuel costs, without any control for carbon emissions. However, we submit that storage may provide necessary flexibility in carbon emission reduction even without carbon tax. We identify the non-convex structure to conduct storage control for this task and propose an easy to implement dynamic programming algorithm to investigate the value of storage in carbon emission reduction.

==> originalproof.tex <==

Define 
$$\bar{\mu}_i(s)\!\coloneqq\! \min_{k\delta \in R^{s}_{i-1}} \big\{\mathbb{E}\{C(s\!-\!k\delta\!+\!D_i)\}+\mu_{i\!-\!1}(k\delta)\big\}$$ $$h_i^s(s')\coloneqq \mathbb{E}\{C(s-s'+D_i)\}+\mu_{i-1}(s')$$
Since $0\le \dot C(\cdot),\dot \mu_{\tau}(\cdot)\le \Bar{M}_c$, so $\big|\dot h_i^s(s')\big|\le \Bar{M}_c$.

Define
$$s^*\coloneqq arg\min_{s'\in R_{i-1}^s}h_i^s(s'),\quad k^*\delta\coloneqq arg\min_{k\delta\in R_{i-1}^s}h_i^s(k\delta)$$
It is obvious $\bar{\mu}_i(s)=h_i^s(k^*\delta)\ge h_i^s(s^*)=\mu_i(s)$. 

Denote  $k'\coloneqq arg \min\{|s^*-k\delta|\big|k\delta\in R_{i-1}^s\}$, then $|s^*-k'\delta|< \delta$.  Then
$$\bar{\mu}_i(s)-\mu_i(s)=h_i^s(k^*\delta)-h_i^s(s^*)\le h_i^s(k'\delta)- h_i^s(s^*)\le \Bar{M}_c\delta$$.  

since $\Tilde{\mu}_i(s)=\min_{k\delta \in R^{s}_{i-1}}\big\{ \mathbb{E}\{C(s-k\delta+D_i)\}+\Tilde{\mu}_{i-1}(k\delta)\big\}$, we know 
\begin{equation*}
    \big|\bar{\mu}_i(s)-\Tilde{\mu}_i(s)\big|
    \le \min_{k\delta \in R^{s}_{i-1}} \big\{\Tilde{\mu}_{i-1}(k\delta)-\mu_{i-1}(k\delta)\}
    \le \bar{M}_c\cdot(i-1)\cdot\delta
\end{equation*}
Then
\begin{align*}
    &\big|\mu_i(s)-\Tilde{\mu}_i(s)\big|\\
    \le& \big|\mu_i(s)-\bar{\mu}_i(s)\big|+\big|\bar{\mu}_i(s)-\Tilde{\mu}_i(s)\big|\\
    \le& \Bar{M}_c\delta+\bar{M}_c\cdot (i-1)\cdot\delta=\bar{M}_c\cdot i\cdot\delta
\end{align*}
Now the Lemma \ref{lemma} get proved.

\emph{Proof of the \textbf{Fact}:}
We prove the fact by induction. 

The induction basis is when $\tau=1$: $\mu_{1}(s)=\mathbb{E}\{C(s-s_0+D_1)\}$. $\dot \mu_{1}(s)\le \Bar{M}_c$ due to the maximal derivative of $C(\cdot)$ is $\Bar{M}_c$. The fact holds. 

Suppose $\dot \mu_{\tau}(s)\le \bar{M}_c$ holds when $\tau=1,...,i-1$. Since $\mu_i(s)=\min_{s'\in R^s_{i-1}}h_i^s(s')$. Here $R^s_{i-1}=R_{i-1}\cap[s+D_i-X,s+D_i]$ where $R_{i-1}$ is the feasible region for $s'$ in $OPT(i-1,s',B)$. By the same way, $\mu_i(s+\Delta s)=\min_{s'\in R^{s+\Delta s}_{i-1}}h_i^{s+\Delta s}(s')$.

Define $\Tilde{s}'$
% For a small quantity $\Delta s>0$, ,$\Tilde{s}''$ 
as following:
$$\Tilde{s}'=arg\min_{s'\in R^s_{i-1}}h_i^s(s')$$
% $$\Tilde{s}''=arg\min_{s'\in R^{s+\Delta s}_{i-1}}h_i^{s+\Delta s}(s')$$

\emph{\textbf{Case} a:} If $\Tilde{s}'\in R^{s}_{i-1}\cap R^{s+\Delta s}_{i-1}$:
\begin{align*}
    &\mu_{i}(s+\Delta s)-\mu_{i}(s)\\
    =&\min_{s'\in R^{s+\Delta s}_{i-1}}h_i^{s+\Delta s}(s')-h_i^{s}(\Tilde{s}')\\
    \le&h_i^{s+\Delta s}(\Tilde{s}')-h_i^{s}(\Tilde{s}')\\
    =&\mathbb{E}\{C(s+\Delta s -\Tilde{s}'+D_{i})\}-\mathbb{E}\{C(s+ -\Tilde{s}'+D_{i})\}\\
    \le &\bar{M}_c\cdot\Delta s
\end{align*}

\emph{\textbf{Case} b:} If $\Tilde{s}'\in R^{s}_{i-1}\verb|\| R^{s+\Delta s}_{i-1}$:
$$R^{s}_{i-1}\verb|\| R^{s+\Delta s}_{i-1}= [s+D_i-X,s+\Delta s+D_i-X)\cap R_{i-1}$$
Denote the lower bound of $R_{i-1}$ as $LR$. If $s+D_i-X<LR$, we can chose $\Delta s$ small enough to make $R^{s}_{i-1}\verb|\| R^{s+\Delta s}_{i-1}=\varnothing$. If $s+D_i-X\ge LR$, we can chose $\Delta s$ small enough to make $R^{s}_{i-1}\verb|\| R^{s+\Delta s}_{i-1}=[s+D_i-X,s+\Delta s+D_i-X)$ and to make $h_i^s(s')$ monotonic in $R^{s}_{i-1}\verb|\| R^{s+\Delta s}_{i-1}$. Then $\Tilde{s}'=s+D_{\tau}-X$.
\begin{align*}
    &\mu_{i}(s+\Delta s)-\mu_{i}(s)\\
    \le &\mu_{i}(s+\Delta s)-\mathbb{E}\{C(X)\}-\mu_{i-1}(s+D_{i}-X)\\
    \le &\mu_{i-1}(s+D_{i}-X+\Delta s)-\mu_{i-1}(s+D_{i}-X)\\
    \le &\bar{M}_c\cdot\Delta s
\end{align*}
Now the fact gets proved.

% When $\tau=1$, $\mu_{1}(s)=\mathbb{E}\{C(s-s_0+D_1)\}$. Since $C(\cdot)$ is non-decreasing, $0\le \dot \mu_{1}(s)$. The fact holds. 
% Suppose $0\le \dot \mu_{\tau}(s)$ holds for $\tau\in\{1,...i\}$.
% Denot $\Tilde{s}'$
% \begin{align*}
%     \mu_{i}(s)=&\min_{s'\in R^{s}_{i-1}}\big\{\mathbb{E}\{C(s-s'+D_{i})\}+\mu_{i-1}(s')\big\}\\
%     =&\mathbb{E}\{C(s-\Tilde{s}'+D_{i})\}+\mu_{i-1}(\Tilde{s}')
% \end{align*}
% \begin{align*}
%     \mu_{i}(s+\Delta s)=&\min_{s'\in R^{s+\Delta s}_{i-1}}}\big\{\mathbb{E}\{C(s+\Delta s-s'+D_{i})\}+\mu_{i-1}(s')\big\}\\
%     =&\mathbb{E}\{C(s+\Delta s -\Tilde{s}''+D_{i})\}+\mu_{i-1}(\Tilde{s}'')
% \end{align*}

% Since $0\le s-s'+D_{i}\le \bar{X}$, and $0\le s'\le B$, then $R^{s}_{i-1}=[\{s+D_i-\bar{X}\}^{+},\{s+D_i -B\}^-+B]$. 

% \emph{a:} If $\Tilde{s}''\in R{'}\cap R^{s+\Delta s}_{i-1}}$, we have $\mu_{i}(s+\Delta s)>\mu_{i}(s)$. 

% \emph{b:} If $\Tilde{s}''\in R{'}\verb|\| R^{s+\Delta s}_{i-1}}$, $\Delta s$ can be small enough, so $R{'}\verb|\| R^{s+\Delta s}_{i-1}}=(s+D_{i},s+\Delta s+D_{i}]$ and $\mathbb{E}\{C(s+\Delta -s'+D_{i})+\mu_{i-1}(s'')\}$ is monotonic when $s'{'}\in R{'}\verb|\| R^{s+\Delta s}_{i-1}}$ which drives $\Tilde{s}''=s+\Delta s+D_{i}$. Then $\mu_{i}(s+\Delta s)=\mu_{i-1}(s+\Delta s)$. Because
% \begin{align*}
%     \mu_{i}(s)=&\min_{s'\in R^{s}_{i-1}}\big\{\mathbb{E}\{C(s-s'+D_{i})\}+\mu_{i-1}(s')\big\}\\
%     \le &\mu_{i-1}(s)\\
%     \le &\mu_{i-1}(s+\Delta s)\\
%     =&\mu_{i}(s+\Delta s)
% \end{align*}
% So $0\le \dot \mu_{\tau}(s)$ holds for $\tau=i$.
% \emph{\textbf{Case} a:} If $\Tilde{s}'\in R^{s}_{i-1}\cap R^{s+\Delta s}_{i-1}$:
% \begin{align*}
%     &\mu_{i}(s+\Delta s)-\mu_{i}(s)\\
%     =&\min_{s'\in R^{s+\Delta s}_{i-1}}\big\{\mathbb{E}\{C(s+\Delta s-s'+D_{i})\}+\mu_{i-1}(s')\big\}-\mu_{i}(s)\\
%     \le &\mathbb{E}\{C(s+\Delta s -\Tilde{s}'+D_{i})\}+\mu_{i-1}(\Tilde{s}')-\mu_{i}(s)\\
%     =&\mathbb{E}\{C(s+\Delta s -\Tilde{s}'+D_{i})\}-\mathbb{E}\{C(s+ -\Tilde{s}'+D_{i})\}\\
%     \le &\bar{M}_c\cdot\Delta s
% \end{align*}


% Suppose $\mu_{\tau}(s)$ is the corresponding optimal objective, $\Tilde{\mu}_{\tau}(s)$ is the result of Algorithm \ref{alg}, i.e. the optimal objective after discretization. Lemma \ref{lemma} claims: $$\big|\mu_{\tau}(s)-\Tilde{\mu}_{\tau}(s)\big|\le \frac{1}{2}\Bar{M}_c\cdot\tau\cdot\delta$$ where $\delta$ is the size of each step and $\Bar{M}_c$ is the maximal derivative of $C(\cdot)$.

% \emph{Proof:}
%  Define $\bar{\mu}_i(s)\!\coloneqq\! \min_{k\delta \in R^{s}_{i-1}} \big\{\mathbb{E}\{C(s\!-\!k\delta\!+\!D_i)\}+\mu_{i\!-\!1}(k\delta)\big\}$. By \textbf{Fact}, $\big|\mu_i(s)\!-\!\bar{\mu}_i(s)\big|\le \frac{1}{2}\bar{M}_c\cdot\delta$.
 
%  When $\tau=1$, $\big|\mu_{1}(s)-\Tilde{\mu}_{1}(s)\big |=0$, Lemma \ref{lemma} holds. 

% Suppose Lemma \ref{lemma} holds for $\tau\in\{1,...,i-1\}$.
% Since $\Tilde{\mu}_i(s)=\min_{k\delta \in R^{s}_{i-1}}\big\{ \mathbb{E}\{C(s-k\delta+D_i)\}+\Tilde{\mu}_{i-1}(k\delta)\big\}$, so
% \begin{equation*}
%     \big|\bar{\mu}_i(s)-\Tilde{\mu}_i(s)\big|
%     \le \min_{k\delta \in R^{s}_{i-1}} \big\{\Tilde{\mu}_{i-1}(k\delta)-\mu_{i-1}(k\delta)\}
%     \le \frac{1}{2}\bar{M}_c\cdot(i-1)\cdot\delta
% \end{equation*}

% Then, $\big|\mu_i(s)-\Tilde{\mu}_i(s)\big|\le \big|\mu_i(s)-\bar{\mu}_i(s)\big|+\big|\bar{\mu}_i(s)-\Tilde{\mu}_i(s)\big|\le \frac{1}{2}\bar{M}_c\cdot i\cdot\delta$. Lemma \ref{lemma} now is proved.



